Greedy Minimum-Energy Scheduling

We consider the problem of energy-efficient scheduling across multiple processors with a power-down mechanism. In this setting a set of $n$ jobs with individual release times, deadlines, and processing volumes must be scheduled across $m$ parallel processors while minimizing the consumed energy. Idle processors can be turned off to save energy, while turning them on requires a fixed amount of energy. For the special case of a single processor, the greedy Left-to-Right algorithm guarantees an approximation factor of $2$. We generalize this simple greedy policy to the case of $m \geq 1$ processors running in parallel and show that the energy costs are still bounded by $2 \text{OPT} + P$, where $\text{OPT}$ is the energy consumed by an optimal solution and $P < \text{OPT}$ is the total processing volume. Our algorithm has a running time of $\mathcal{O}(n f \log d)$, where $d$ is the difference between the latest deadline and the earliest release time, and $f$ is the running time of a maximum flow calculation in a network of $\mathcal{O}(n)$ nodes.

==> graphics/constellation <==
<mxfile host="app.diagrams.net" modified="2023-04-23T18:15:36.399Z" agent="Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/111.0.0.0 Safari/537.36" etag="x119wFTll3nVGz8TEA_o" version="21.2.1" type="device">
  <diagram name="8.1" id="HRK91SzV57C4mrXLqSAv">
    <mxGraphModel dx="1562" dy="837" grid="0" gridSize="50" guides="1" tooltips="1" connect="1" arrows="0" fold="1" page="1" pageScale="1" pageWidth="1600" pageHeight="900" math="1" shadow="0">
      <root>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-0" />
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-1" parent="mwbZKrUk0B2fcWtcdBXQ-0" />
        <mxCell id="erL9w4hDm6DtMNve198--0" value="$$j$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="916" y="451" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-5" value="$$S^1_{\mathrm{aug}}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="352" y="450" width="300" height="50" as="geometry" />
        </mxCell>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-6" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="501" y="450" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-7" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="901" y="450" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-9" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=ERone;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;strokeColor=#000000;" parent="mwbZKrUk0B2fcWtcdBXQ-1" source="mwbZKrUk0B2fcWtcdBXQ-6" target="mwbZKrUk0B2fcWtcdBXQ-7" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="801" y="398" as="sourcePoint" />
            <mxPoint x="801" y="448" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-12" value="&lt;div style=&quot;font-size: 25px&quot;&gt;&lt;br&gt;&lt;/div&gt;" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="679" y="401" width="50" height="50" as="geometry" />
        </mxCell>
        <mxCell id="cCJ7NgLmofpjaUjCZAvd-4" value="$$A_r$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="982" y="400" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="cCJ7NgLmofpjaUjCZAvd-5" value="\(I\)" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="794" y="401" width="50" height="50" as="geometry" />
        </mxCell>
        <mxCell id="erL9w4hDm6DtMNve198--1" value="$$A_l$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="581" y="400" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="UghbR5yeUCLeYgXvmuru-1" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=1;exitY=0.5;exitDx=0;exitDy=0;strokeColor=#000000;" parent="mwbZKrUk0B2fcWtcdBXQ-1" source="mwbZKrUk0B2fcWtcdBXQ-7" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="751" y="525" as="sourcePoint" />
            <mxPoint x="1155" y="475" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="so3PqimSafIuxcuDGIZe-0" value="$$j$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="910" y="452" width="79" height="42" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> graphics/engagements <==
<mxfile host="app.diagrams.net" modified="2023-04-23T17:45:39.173Z" agent="Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/111.0.0.0 Safari/537.36" etag="g00IGN6pMsoHGXbxWlK3" version="21.2.1" type="device">
  <diagram name="8.1" id="HRK91SzV57C4mrXLqSAv">
    <mxGraphModel dx="1838" dy="985" grid="1" gridSize="25" guides="1" tooltips="1" connect="1" arrows="0" fold="1" page="1" pageScale="1" pageWidth="1600" pageHeight="900" math="1" shadow="0">
      <root>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-0" />
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-1" parent="mwbZKrUk0B2fcWtcdBXQ-0" />
        <mxCell id="yPNepUL52WUj2P0wk5Aj-1" value="$$S^{k&#39;}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="401" y="598.82" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-15" value="$$S^k$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="401" y="498.82" width="125" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-16" value="$$S^{k&#39;}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="401" y="400" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-17" value="" style="shape=curlyBracket;whiteSpace=wrap;html=1;rounded=1;labelPosition=left;verticalLabelPosition=middle;align=right;verticalAlign=middle;strokeColor=#000000;fillColor=default;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="374" y="498.82" width="20" height="150" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-18" value="Before close" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="199" y="549.82" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-19" value="After close" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="200" y="400" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-12" value="" style="group" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1" connectable="0">
          <mxGeometry x="500" y="400" width="100" height="250" as="geometry" />
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-0" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=0;exitY=0.5;exitDx=0;exitDy=0;" parent="S7Po_t00T9Il-vt3TeZs-12" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="50" y="24.409999999999968" as="sourcePoint" />
            <mxPoint y="24" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-2" value="$$t$$" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;strokeColor=none;" parent="S7Po_t00T9Il-vt3TeZs-12" vertex="1">
          <mxGeometry x="50" width="50" height="50" as="geometry" />
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-3" value="" style="endArrow=none;html=1;strokeWidth=2;" parent="S7Po_t00T9Il-vt3TeZs-12" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="50" as="sourcePoint" />
            <mxPoint x="100" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-4" value="" style="endArrow=none;html=1;strokeWidth=2;entryX=0;entryY=1;entryDx=0;entryDy=0;" parent="S7Po_t00T9Il-vt3TeZs-12" target="S7Po_t00T9Il-vt3TeZs-2" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="50" as="sourcePoint" />
            <mxPoint x="150" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-5" value="" style="endArrow=none;html=1;strokeWidth=2;exitX=0;exitY=1;exitDx=0;exitDy=0;" parent="S7Po_t00T9Il-vt3TeZs-12" source="S7Po_t00T9Il-vt3TeZs-2" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="100" y="50" as="sourcePoint" />
            <mxPoint x="100" y="50" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-6" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=none;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=0;exitY=0.5;exitDx=0;exitDy=0;" parent="S7Po_t00T9Il-vt3TeZs-12" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="50" y="123.22999999999996" as="sourcePoint" />
            <mxPoint y="122.82" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-11" value="" style="group" parent="S7Po_t00T9Il-vt3TeZs-12" vertex="1" connectable="0">
          <mxGeometry y="198.82" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-7" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;strokeColor=none;" parent="S7Po_t00T9Il-vt3TeZs-11" vertex="1">
          <mxGeometry width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-8" value="" style="endArrow=none;html=1;strokeWidth=2;" parent="S7Po_t00T9Il-vt3TeZs-11" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint as="sourcePoint" />
            <mxPoint x="100" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-10" value="" style="endArrow=none;html=1;strokeWidth=2;exitX=0;exitY=1;exitDx=0;exitDy=0;" parent="S7Po_t00T9Il-vt3TeZs-11" source="S7Po_t00T9Il-vt3TeZs-7" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="100" y="50" as="sourcePoint" />
            <mxPoint x="100" y="50" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="S7Po_t00T9Il-vt3TeZs-13" value="$$\ldots$$" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="S7Po_t00T9Il-vt3TeZs-12" vertex="1">
          <mxGeometry x="-44" y="142.82" width="125" height="50" as="geometry" />
        </mxCell>
        <mxCell id="bOvuwz93vkdH_OUuYojW-0" value="$$\ldots$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="S7Po_t00T9Il-vt3TeZs-12" vertex="1">
          <mxGeometry x="-99" y="143.82000000000005" width="125" height="50" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> graphics/invariant_case1 <==
<mxfile host="app.diagrams.net" modified="2023-04-23T17:57:14.790Z" agent="Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/111.0.0.0 Safari/537.36" etag="51Flzyo2TvrWkjzcJxBD" version="21.2.1" type="device">
  <diagram name="8.1" id="HRK91SzV57C4mrXLqSAv">
    <mxGraphModel dx="1562" dy="837" grid="1" gridSize="50" guides="1" tooltips="1" connect="1" arrows="0" fold="1" page="1" pageScale="1" pageWidth="1600" pageHeight="900" math="1" shadow="0">
      <root>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-0" />
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-1" parent="mwbZKrUk0B2fcWtcdBXQ-0" />
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-21" value="$$B&#39;&#39;$$" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;strokeColor=none;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="800" y="200" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="yPNepUL52WUj2P0wk5Aj-1" value="$$k&#39;_V$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="401" y="250" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-0" value="" style="group" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1" connectable="0">
          <mxGeometry x="550" y="250" width="485" height="51" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-0" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;strokeColor=none;" parent="NlHelRNHxiFcZa0GTOFG-0" vertex="1">
          <mxGeometry y="1" width="484.46170921198666" height="50" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-5" value="" style="endArrow=none;html=1;strokeWidth=2;entryX=1;entryY=0;entryDx=0;entryDy=0;" parent="NlHelRNHxiFcZa0GTOFG-0" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint y="51" as="sourcePoint" />
            <mxPoint x="484.46170921198666" y="51" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-8" value="" style="endArrow=none;html=1;strokeWidth=2;entryX=1;entryY=0;entryDx=0;entryDy=0;" parent="NlHelRNHxiFcZa0GTOFG-0" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="0.5382907880133185" as="sourcePoint" />
            <mxPoint x="485" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-7" value="" style="endArrow=none;html=1;rounded=0;strokeWidth=2;" parent="NlHelRNHxiFcZa0GTOFG-0" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="484.46535433070864" y="51" as="sourcePoint" />
            <mxPoint x="484.46535433070864" y="1" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-10" value="$$B$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="NlHelRNHxiFcZa0GTOFG-0" vertex="1">
          <mxGeometry x="284.0028346456693" y="1" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-14" value="" style="endArrow=none;html=1;strokeWidth=2;" parent="NlHelRNHxiFcZa0GTOFG-0" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="305.51181102362204" as="sourcePoint" />
            <mxPoint x="381.8897637795275" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-5" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=0;exitY=0.5;exitDx=0;exitDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" source="Yu52MZWXu-L9lN7ZfvFl-21" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="350" y="200.28999999999996" as="sourcePoint" />
            <mxPoint x="650" y="225" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-8" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="1035" y="275.21" as="sourcePoint" />
            <mxPoint x="1100" y="275" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-9" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=none;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="1035" y="226.70999999999998" as="sourcePoint" />
            <mxPoint x="1100" y="226.5" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-11" value="$$B&#39;$$" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="800" y="400" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-12" value="" style="endArrow=none;html=1;strokeWidth=2;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="800" y="200" as="sourcePoint" />
            <mxPoint x="900" y="200" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-13" value="" style="endArrow=none;html=1;strokeWidth=2;entryX=0;entryY=1;entryDx=0;entryDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" target="Yu52MZWXu-L9lN7ZfvFl-21" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="800" y="200" as="sourcePoint" />
            <mxPoint x="900" y="200" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-15" value="$$k&#39;_V + 1$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="401" y="200" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-16" value="$$k&#39;_V$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="401" y="400" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-17" value="" style="shape=curlyBracket;whiteSpace=wrap;html=1;rounded=1;labelPosition=left;verticalLabelPosition=middle;align=right;verticalAlign=middle;strokeColor=#000000;fillColor=default;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="374" y="200" width="20" height="100" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-18" value="Before close" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="199" y="225" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-19" value="After close" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="199" y="400" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-20" value="" style="shape=curlyBracket;whiteSpace=wrap;html=1;rounded=1;labelPosition=left;verticalLabelPosition=middle;align=right;verticalAlign=middle;strokeColor=#000000;fillColor=default;rotation=90;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="875.5" y="-118.5" width="20" height="571" as="geometry" />
        </mxCell>
        <mxCell id="NlHelRNHxiFcZa0GTOFG-21" value="$$\text{Valley } V$$" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="756" y="88" width="250" height="50" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> graphics/lemma_intersection <==
<mxfile host="app.diagrams.net" modified="2023-04-23T18:08:39.151Z" agent="Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/111.0.0.0 Safari/537.36" etag="jBVBU-jp4Cr9gksMbmYv" version="21.2.1" type="device">
  <diagram name="8.3" id="03_SKRS_E9v-FVpuEGA3">
    <mxGraphModel dx="1562" dy="837" grid="1" gridSize="50" guides="1" tooltips="1" connect="1" arrows="0" fold="1" page="1" pageScale="1" pageWidth="1600" pageHeight="900" math="1" shadow="0">
      <root>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-0" />
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-1" parent="FHt6qTQTZ3OI_9cPNjQw-0" />
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-4" value="" style="group" parent="FHt6qTQTZ3OI_9cPNjQw-1" vertex="1" connectable="0">
          <mxGeometry x="201" y="401" width="1100" height="249" as="geometry" />
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-5" value="$$S^k_{ltr}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="FHt6qTQTZ3OI_9cPNjQw-4" vertex="1">
          <mxGeometry y="53" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-6" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="FHt6qTQTZ3OI_9cPNjQw-4" vertex="1">
          <mxGeometry x="300" y="49" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-7" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="FHt6qTQTZ3OI_9cPNjQw-4" vertex="1">
          <mxGeometry x="700" y="49" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-8" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=ERone;endFill=0;verticalAlign=middle;exitX=1;exitY=0.5;exitDx=0;exitDy=0;strokeWidth=4;fillColor=#e3c800;strokeColor=#000000;" parent="FHt6qTQTZ3OI_9cPNjQw-4" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="100" y="74.70999999999975" as="sourcePoint" />
            <mxPoint x="300" y="74" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-9" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=ERone;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#e3c800;strokeColor=#000000;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;" parent="FHt6qTQTZ3OI_9cPNjQw-4" source="FHt6qTQTZ3OI_9cPNjQw-6" target="FHt6qTQTZ3OI_9cPNjQw-7" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="600" y="-3" as="sourcePoint" />
            <mxPoint x="600" y="47" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-10" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=ERone;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#e3c800;strokeColor=#000000;exitX=1;exitY=0.5;exitDx=0;exitDy=0;" parent="FHt6qTQTZ3OI_9cPNjQw-4" source="FHt6qTQTZ3OI_9cPNjQw-7" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="950" y="73.65999999999997" as="sourcePoint" />
            <mxPoint x="1100" y="74" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-11" value="&lt;div style=&quot;font-size: 25px&quot;&gt;&lt;font style=&quot;font-size: 25px&quot;&gt;$$S^k_{opt}$$&lt;/font&gt;&lt;/div&gt;" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=30;" parent="FHt6qTQTZ3OI_9cPNjQw-4" vertex="1">
          <mxGeometry y="199" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-15" value="\( S_{opt} \) requires \(k\) processors" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="FHt6qTQTZ3OI_9cPNjQw-4" vertex="1">
          <mxGeometry x="474" y="149" width="450" height="50" as="geometry" />
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-16" value="&lt;div&gt;&lt;br&gt;&lt;/div&gt;&lt;div&gt;&lt;br&gt;&lt;/div&gt;" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=ERone;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f8cecc;strokeColor=#000000;" parent="FHt6qTQTZ3OI_9cPNjQw-1" edge="1">
          <mxGeometry y="198.65999999999997" as="geometry">
            <mxPoint x="451" y="624.6599999999999" as="sourcePoint" />
            <mxPoint x="1151" y="624.6599999999999" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="FHt6qTQTZ3OI_9cPNjQw-17" value="" style="shape=curlyBracket;whiteSpace=wrap;html=1;rounded=1;flipH=1;fontSize=25;fillColor=none;align=center;rotation=90;" parent="FHt6qTQTZ3OI_9cPNjQw-1" vertex="1">
          <mxGeometry x="885" y="338.5" width="30" height="400" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> graphics/running_time <==
<mxfile host="app.diagrams.net" modified="2023-04-23T18:20:16.163Z" agent="Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/111.0.0.0 Safari/537.36" etag="OHZXIwR11EXiRWR1_tA-" version="21.2.1" type="device">
  <diagram name="8.1" id="HRK91SzV57C4mrXLqSAv">
    <mxGraphModel dx="1562" dy="837" grid="1" gridSize="50" guides="1" tooltips="1" connect="1" arrows="0" fold="1" page="1" pageScale="1" pageWidth="1600" pageHeight="900" math="1" shadow="0">
      <root>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-0" />
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-1" parent="mwbZKrUk0B2fcWtcdBXQ-0" />
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-0" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;strokeColor=none;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="300" y="750" width="900" height="50" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-4" value="" style="endArrow=none;html=1;strokeWidth=2;entryX=1;entryY=0;entryDx=0;entryDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" target="Yu52MZWXu-L9lN7ZfvFl-0" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="300" y="750" as="sourcePoint" />
            <mxPoint x="350" y="700" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-5" value="" style="endArrow=none;html=1;strokeWidth=2;entryX=1;entryY=0;entryDx=0;entryDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="300" y="800" as="sourcePoint" />
            <mxPoint x="1200" y="800" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-6" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;strokeColor=none;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="301" y="701" width="900" height="50" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-7" value="" style="endArrow=none;html=1;strokeWidth=2;entryX=1;entryY=0;entryDx=0;entryDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" target="Yu52MZWXu-L9lN7ZfvFl-6" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="301" y="699" as="sourcePoint" />
            <mxPoint x="351" y="649" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-8" value="" style="endArrow=none;html=1;strokeWidth=2;entryX=1;entryY=0;entryDx=0;entryDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry width="50" height="50" relative="1" as="geometry">
            <mxPoint x="301" y="749" as="sourcePoint" />
            <mxPoint x="1201" y="749" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="mwbZKrUk0B2fcWtcdBXQ-5" value="$$S^1_{\mathrm{pltr}}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="200" y="751" width="300" height="50" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-18" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="301" y="550" width="899" height="50" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-19" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="500" y="500" width="610" height="50" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-20" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="850" y="450" width="220" height="50" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-21" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeWidth=2;fontColor=#333333;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="900" y="400" width="110" height="50" as="geometry" />
        </mxCell>
        <mxCell id="Yu52MZWXu-L9lN7ZfvFl-22" value="$$B&#39;$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="937" y="352" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="yPNepUL52WUj2P0wk5Aj-0" value="$$S^k_{\mathrm{pltr}}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="200" y="550" width="300" height="50" as="geometry" />
        </mxCell>
        <mxCell id="yPNepUL52WUj2P0wk5Aj-1" value="$$S^l_{\mathrm{pltr}}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="200" y="400" width="300" height="50" as="geometry" />
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-0" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=1;exitY=0.5;exitDx=0;exitDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="1010" y="424.29" as="sourcePoint" />
            <mxPoint x="1250" y="424" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-2" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=1;exitY=0.5;exitDx=0;exitDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="1070" y="474.78999999999996" as="sourcePoint" />
            <mxPoint x="1250" y="475" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-3" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=1;exitY=0.5;exitDx=0;exitDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="1110" y="524.79" as="sourcePoint" />
            <mxPoint x="1250" y="525" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-4" style="edgeStyle=none;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;fontSize=15;startArrow=ERone;startFill=0;endArrow=none;endFill=0;verticalAlign=middle;strokeWidth=4;fillColor=#f5f5f5;exitX=1;exitY=0.5;exitDx=0;exitDy=0;" parent="mwbZKrUk0B2fcWtcdBXQ-1" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="1201" y="574.79" as="sourcePoint" />
            <mxPoint x="1250" y="575" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-5" value="$$B$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="784" y="550" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-7" value="$$j_1$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="910" y="751" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-8" value="$$j_2$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="910" y="700" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-9" value="$$j_k$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="907" y="550" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-10" value="$$j_l$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="910" y="400" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-11" value="$$\ldots$$" style="text;html=1;align=center;verticalAlign=middle;resizable=0;points=[];autosize=1;fontSize=40;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="695" y="612" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-12" value="$$j_{k+1}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="907" y="500" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="n6zg_OlYmCGUuVlRfv8S-13" value="$$j_{l-1}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="mwbZKrUk0B2fcWtcdBXQ-1" vertex="1">
          <mxGeometry x="910" y="450" width="150" height="50" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> graphics/valleys_of <==
<mxfile host="app.diagrams.net" modified="2023-04-23T18:00:38.229Z" agent="Mozilla/5.0 (X11; Linux x86_64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/111.0.0.0 Safari/537.36" etag="4r-tQ_Y_I1nbfu4xZHTl" version="21.2.1" type="device">
  <diagram id="35FyVSaM5qYDxZm-93JJ" name="Page-2">
    <mxGraphModel dx="2603" dy="1395" grid="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" page="1" pageScale="1" pageWidth="850" pageHeight="1100" math="1" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="KUlynp-E6a5BVeWY_m1j-33" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="200" y="550" width="1650" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-34" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="300" y="450" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-35" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="550" y="450" width="350" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-36" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="600" y="400" width="250" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-37" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="650" y="350" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-38" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="700" y="300" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-39" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="1200" y="450" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-40" value="$$S^k_{\mathrm{pltr}}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="1" vertex="1">
          <mxGeometry x="50" y="450" width="300" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-41" value="$$S^1_{\mathrm{pltr}}$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="1" vertex="1">
          <mxGeometry x="50" y="600" width="300" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-42" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="250" y="500" width="650" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-43" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="1000" y="500" width="350" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-44" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="1400" y="500" width="400" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-45" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="1450" y="450" width="300" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-46" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="1500" y="400" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-47" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="1550" y="350" width="100" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-48" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#f5f5f5;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="1" vertex="1">
          <mxGeometry x="200" y="600" width="1650" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-49" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="50" y="664" width="1700" height="136" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-10" value="$$C_k:$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry y="86" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-11" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#FFFFFF;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="200" y="86" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-12" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#FFFFFF;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="500" y="86" width="250" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-13" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#FFFFFF;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="1050" y="86" width="200" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-14" value="$$D_1$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="279" y="86" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-15" value="$$D_2$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="600" y="86" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-16" value="$$D_3$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="1132" y="86" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-19" value="$$V_1$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="432" y="5" width="120" height="40" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-20" value="" style="strokeWidth=2;html=1;shape=mxgraph.flowchart.annotation_2;align=left;labelPosition=right;pointerEvents=1;fillColor=#FFFFFF;rotation=90;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="432" y="11" width="36" height="100" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-21" value="" style="strokeWidth=2;html=1;shape=mxgraph.flowchart.annotation_2;align=left;labelPosition=right;pointerEvents=1;fillColor=#FFFFFF;rotation=90;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="882" y="-88" width="36" height="300" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-22" value="$$V_2$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="886" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-27" value="" style="rounded=0;whiteSpace=wrap;html=1;fontSize=25;fillColor=#FFFFFF;strokeColor=#000000;strokeWidth=2;fontColor=#333333;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="1400" y="86" width="300" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-28" value="$$D_4$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="1536" y="86" width="150" height="50" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-29" value="$$V_3$$" style="text;html=1;align=left;verticalAlign=middle;resizable=0;points=[];autosize=1;strokeColor=none;fillColor=none;fontSize=25;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="1308" y="5" width="120" height="40" as="geometry" />
        </mxCell>
        <mxCell id="KUlynp-E6a5BVeWY_m1j-30" value="" style="strokeWidth=2;html=1;shape=mxgraph.flowchart.annotation_2;align=left;labelPosition=right;pointerEvents=1;fillColor=#FFFFFF;rotation=90;" parent="KUlynp-E6a5BVeWY_m1j-49" vertex="1">
          <mxGeometry x="1307" y="-13" width="36" height="150" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>

